A Least-Squares-Based Neural Network (LS-Net) for Solving Linear Parametric PDEs

Developing efficient methods for solving parametric partial differential equations is crucial for addressing inverse problems. This work introduces a Least-Squares-based Neural Network (LS-Net) method for solving linear parametric PDEs. It utilizes a separated representation form for the parametric PDE solution via a deep neural network and a least-squares solver. In this approach, the output of the deep neural network consists of a vector-valued function, interpreted as basis functions for the parametric solution space, and the least-squares solver determines the optimal solution within the constructed solution space for each given parameter. The LS-Net method requires a quadratic loss function for the least-squares solver to find optimal solutions given the set of basis functions. In this study, we consider loss functions derived from the Deep Fourier Residual and Physics-Informed Neural Networks approaches. We also provide theoretical results similar to the Universal Approximation Theorem, stating that there exists a sufficiently large neural network that can theoretically approximate solutions of parametric PDEs with the desired accuracy. We illustrate the LS-net method by solving one- and two-dimensional problems. Numerical results clearly demonstrate the method's ability to approximate parametric solutions.

==> Figure_DeepONet.tex <==
\begin{tikzpicture}[
punkt/.style={
   rectangle,
   rounded corners,
   draw=black, thick,
   text width=2em,
   minimum height=1em,
   text centered}
]
% The Trunk net %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\draw (2,1.5) node{ $x \rightarrow$};
\node[punkt, minimum width = 12.8em, minimum height = 10em, dashed, blue] (block) at (3.8, 1.5) {};
\node[punkt, minimum width = 5.5em, minimum height = 3.5em] (block) at (3.5, 1.5) {};
\draw [blue] (3.8, 3.5) node{Trunk net};
\draw (3.5, 1.7) node{A single};
\draw (3.5, 1.3) node{layer NN};

\node[punkt, minimum width = 1 em, minimum height = 9.4em] (block) at (5.5, 1.5) { };

\Vertex[x=5.5,y=2.7,label=$u_1^\alpha\hspace{-0.05cm}(x)$,color=white,size=0.8,fontsize=\scriptsize]{A11}
\Vertex[x=5.5,y=1.8, label=$u_2^\alpha\hspace{-0.05cm}(x)$,color=white,size=0.8,fontsize=\scriptsize]{A12}
\Vertex[x=5.5,y=0.3, label=$u_N^\alpha\hspace{-0.05cm}(x)$,color=white,size=0.8,fontsize=\scriptsize]{A13}

\Edge[color=red, Direct,lw=0.5pt](4.45, 1.5)(A11)
\Edge[color=red, Direct,lw=0.5pt](4.45, 1.5)(A12)
\Edge[color=red, Direct,lw=0.5pt](4.45, 1.5)(A13)
% The Branch net %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\node[punkt, minimum width = 12.8em, minimum height = 10em, draw, dashed, blue] (block) at (3.8, -2.3) {};

\draw (1.8,-2.3) node{$p$};
\draw (2.2,-2.3) node{ $\rightarrow$};
\node[punkt, minimum width = 5.5em, minimum height = 2em] (block) at (3.5, -2.3) {};
\draw [blue](3.8, -4.3) node{Branch net};
\draw (3.5, -2.3) node{A Deep NN};
\node[punkt, minimum width = 1em, minimum height = 9.4em] (block) at (5.5, -2.3) {};

\Vertex[x=5.5,y=-1.1,label=$c_1\hspace{-0.05cm}(p)$,color=white,size=0.8,fontsize=\scriptsize]{B11}
\Vertex[x=5.5,y=-2, label=$c_2\hspace{-0.03cm}(p)$,color=white,size=0.8,fontsize=\scriptsize]{B12}
\Vertex[x=5.5,y=-3.5, label=$c_N\hspace{-0.05cm}(p)$,color=white,size=0.8,fontsize=\scriptsize]{B13}

\Edge[color=red, Direct,lw=0.5pt](4.45, -2.3)(B11)
\Edge[color=red, Direct,lw=0.5pt](4.45, -2.3)(B12)
\Edge[color=red, Direct,lw=0.5pt](4.45, -2.3)(B13)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\node[punkt, minimum width = 9em, minimum height = 3.5em] (block) at (8.2, -0.2) {};
\draw (8.2, -0.2) node{$\displaystyle \sum _{i = 1}^{N}c_i u_i^\alpha = u^{\alpha, \mathbf{c}}$};
%\Vertex[x = 7,y = -0.2, label=$\sum _{i = 1}^{N} b_i(x)c_i(x)$,color=white,size=0.55,fontsize=\normalsize]{C1}
\Edge[color=red, Direct,lw=0.5pt](6, 1.5)(6.6, 0.4)
\Edge[color=red, Direct,lw=0.5pt](6, -2)(6.6, -0.8)
\end{tikzpicture}

